Differentiable Particle Filtering via Entropy-Regularized Optimal Transport

Particle Filtering (PF) methods are an established class of procedures for performing inference in non-linear state-space models. Resampling is a key ingredient of PF, necessary to obtain low variance likelihood and states estimates. However, traditional resampling methods result in PF-based loss functions being non-differentiable with respect to model and PF parameters. In a variational inference context, resampling also yields high variance gradient estimates of the PF-based evidence lower bound. By leveraging optimal transport ideas, we introduce a principled differentiable particle filter and provide convergence results. We demonstrate this novel method on a variety of applications.

==> Differentiable_Particle_Filter (arXiv)/tables/MULTINOMIAL_batchsize_100_N_100_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -3.296 & 0.078 \\
                  0.500 & -3.136 & 0.062 \\
                  0.750 & -3.228 & 0.068 \\
\bottomrule
\end{tabular}


==> Differentiable_Particle_Filter (arXiv)/tables/MULTINOMIAL_batchsize_100_N_25_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -4.068 & 0.177 \\
                  0.500 & -3.801 & 0.169 \\
                  0.750 & -3.896 & 0.176 \\
\bottomrule
\end{tabular}


==> Differentiable_Particle_Filter (arXiv)/tables/MULTINOMIAL_batchsize_100_N_50_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -3.562 & 0.110 \\
                  0.500 & -3.350 & 0.100 \\
                  0.750 & -3.443 & 0.106 \\
\bottomrule
\end{tabular}


==> Differentiable_Particle_Filter (arXiv)/tables/REGULARIZED_batchsize_100_N_100_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -3.298 & 0.074 \\
                  0.500 & -3.140 & 0.060 \\
                  0.750 & -3.237 & 0.065 \\
\bottomrule
\end{tabular}


==> Differentiable_Particle_Filter (arXiv)/tables/REGULARIZED_batchsize_100_N_25_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -4.071 & 0.180 \\
                  0.500 & -3.806 & 0.172 \\
                  0.750 & -3.896 & 0.180 \\
\bottomrule
\end{tabular}


==> Differentiable_Particle_Filter (arXiv)/tables/REGULARIZED_batchsize_100_N_50_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -3.568 & 0.109 \\
                  0.500 & -3.355 & 0.104 \\
                  0.750 & -3.454 & 0.127 \\
\bottomrule
\end{tabular}


==> Differentiable_Particle_Filter (arXiv)/tables/VARIANCE_CORRECTED_batchsize_100_N_100_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -3.298 & 0.074 \\
                  0.500 & -3.140 & 0.060 \\
                  0.750 & -3.237 & 0.065 \\
\bottomrule
\end{tabular}


==> Differentiable_Particle_Filter (arXiv)/tables/VARIANCE_CORRECTED_batchsize_100_N_25_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -4.072 & 0.181 \\
                  0.500 & -3.807 & 0.172 \\
                  0.750 & -3.894 & 0.178 \\
\bottomrule
\end{tabular}


==> Differentiable_Particle_Filter (arXiv)/tables/VARIANCE_CORRECTED_batchsize_100_N_50_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -3.568 & 0.109 \\
                  0.500 & -3.355 & 0.104 \\
                  0.750 & -3.454 & 0.126 \\
\bottomrule
\end{tabular}


==> Differentiable_Particle_Filter (arXiv)/tables/kalman_likelihoods_values.tex <==
\begin{tabular}{rr}
\toprule
 $\theta_1, \theta_2$ &  $\ell(\theta_1, \theta_2)$ \\
\midrule
                0.250 &                      -3.052 \\
                0.500 &                      -2.958 \\
                0.750 &                      -3.015 \\
\bottomrule
\end{tabular}


==> Differentiable_Particle_Filter (arXiv)/tables/merged_tables/RMSE_optimal_proposal.tex <==

 \begin{tabular}{rrrr}
 \toprule
 & $\ell^\text{ELBO}$ & $\ell^\text{ELBO}_\epsilon$ & $\ell_\epsilon$ \\
 \midrule
  $\text{RMSE}(\phi - \mathbf{1})$ &   0.124 &   0.110 &   0.237\\
 \bottomrule
 \end{tabular}

==> Differentiable_Particle_Filter (arXiv)/tables/merged_tables/elbo_stats.tex <==

%  \begin{tabular}{rrrrrrrrr}
%  \toprule
%   & \multicolumn{2}{c}{PF} & \multicolumn{2}{c}{DPF ($\epsilon=0.25$)} & \multicolumn{2}{c}{DPF ($\epsilon=0.5$)} & \multicolumn{2}{c}{DPF ($\epsilon=0.75$)}\\
% \midrule
%   $\theta_1$, $\theta_2$ &   mean &   std &   mean &   std &   mean &   std &   mean &   std \\
% \midrule
%                   0.25 & -1.13  & 0.20 & -1.14 & 0.20 & -1.14 & 0.20 & -1.14 & 0.20  \\
%                   0.50 & -0.93  & 0.18 & -0.94 & 0.18 & -0.94 & 0.18 & -0.94 & 0.18  \\
%                   0.75 & -1.05 & 0.17 &  -1.07 & 0.19 & -1.08 & 0.18 & -1.08 & 0.18\\
%  \bottomrule
%  \end{tabular}
 
 
 \begin{tabular}{rrrrr}
 \toprule
   \multicolumn{2}{c}{$\theta_1$, $\theta_2$}           & 0.25  & 0.5   & 0.75 \\
   \midrule
   \multirow{2}{*}{PF}                           & mean & -1.13 & -0.93 & -1.05 \\
                                                 & std  & 0.20  & 0.18  & 0.17 \\
   \midrule
   \multirow{2}{*}{DPF ($\epsilon=0.25$)}        & mean & -1.14 & -0.94 & -1.07 \\
                                                 & std  & 0.20  & 0.18  & 0.19 \\
   \midrule
   \multirow{2}{*}{DPF ($\epsilon=0.5$)}         & mean & -1.14 & -0.94 & -1.08 \\
                                                 & std  & 0.20  & 0.18  & 0.18 \\
   \midrule
   \multirow{2}{*}{DPF ($\epsilon=0.75$)}        & mean & -1.14 & -0.94 & -1.08 \\
                                                 & std  & 0.20  & 0.18  & 0.18 \\
 \bottomrule
 \end{tabular}
 
 
 
% OLD dataset! same kind of results, but no eps =.25 or .75 
%   \begin{tabular}{rrrrr}
%  \toprule
%   & \multicolumn{2}{c}{PF} & \multicolumn{2}{c}{DPF}\\
% \midrule
%   $\theta_1$, $\theta_2$ &   mean &   std &   mean &   std \\
% \midrule
%                   0.25 & -1.02  & 0.18 & -1.02 & 0.18  \\
%                   0.50 & -0.84  & 0.17 & -0.85 & 0.17  \\
%                   0.75 & -0.79 & 0.18 &  -0.79 & 0.18 \\
%  \bottomrule
%  \end{tabular}


%  \begin{tabular}{rrrrrr}
%  \toprule
%   & \multicolumn{2}{c}{Multinomial} & \multicolumn{2}{c}{DET} & \begin{tabular}[c]{@{}l@{}}Kalman \\ Filter\end{tabular} \\
% \midrule
%   $\theta_1$, $\theta_2$ &   mean &   std &   mean &   std & $\ell(\theta_1, \theta_2)$ \\
% \midrule
%                   0.250 & -4.068 & 0.177 & -4.071 & 0.180 & -3.052 \\
%                   0.500 & -3.801 & 0.169 & -3.806 & 0.172 & -2.958 \\
%                   0.750 & -3.896 & 0.176 & -3.896 & 0.180 & -3.015 \\
%  \bottomrule
%  \end{tabular}

% likelihood tables for Multinomial 100 25, Regularized 100 25, Kalman

==> Differentiable_Particle_Filter (arXiv)/tables/merged_tables/rmse_with_average_smle.tex <==
\begin{table}[H]
    \centering
        \caption{Root mean square error\footnotemark \\ over 50 datasets $/10^{-3}$ }
        \begin{tabular}{llll}
            \toprule
            & $\hat{\theta}^\text{MUL}_{\text{ELBO}}$ & $\hat{\theta}^\text{DET}_{\text{ELBO}}$ & $\hat{\theta}_{\text{Average SMLE}}$ \\
                       \midrule
            $\theta_1$ & 3.76   & 2.72   & 5.83                         \\
            $\theta_2$ & 3.20   & 2.07   & 4.64     \\ 
            \bottomrule
        \end{tabular}
    \label{tab:theta_diff}
\end{table}


==> Differentiable_Particle_Filter (arXiv)/tables/merged_tables/theta_rmse.tex <==
% \begin{tabular}{lllll}
%             \toprule
%             & $\hat{\theta}^\text{MUL}_{\text{ELBO}}$ & $\hat{\theta}^\text{DET}_{\text{ELBO}}$ & $\hat{\theta}_{\text{ASMLE}}$ & $\hat{\theta}_{\text{SMLE}}$ \\
%                       \midrule
%             $\theta_1$ & 3.76   & 2.72   & 5.83 & 11.9                         \\
%             $\theta_2$ & 3.20   & 2.07   & 4.64 & 12.6    \\ 
%             \bottomrule
%     \end{tabular}

% \begin{tabular}{llll}
% \toprule
% $B$ &  $\hat{\theta}^\text{PF}_{\text{ELBO}}$ & $\hat{\theta}^\text{DPF}_{\text{ELBO}}$ & $\hat{\theta}_{\text{SMLE}}$ \\ \midrule
% 1         & 4.86                 & 3.94                 & 16.87                 \\
% 4          & 4.94                 & 3.37                 & 7.01                  \\
% 10         & 4.79                 & 2.72                 & 4.53                  \\
% 25         & 4.83                 & 2.23                 & 2.74          \\       \bottomrule
% \end{tabular}

\begin{tabular}{llll}
\toprule
$B$ &  $\hat{\theta}^\text{PF}_{\text{ELBO}}$ & $\hat{\theta}^\text{DPF}_{\text{ELBO}}$ & $\hat{\theta}_{\text{SMLE}}$ \\ \midrule
1         & 1.94                 & 1.30                 & 7.94                 \\
4          & 2.40                 & 1.35                 & 3.28                  \\
10         & 2.80                 & 1.37                & 2.18                  \\
\bottomrule
\end{tabular}

==> Differentiable_Particle_Filter (arXiv)/tables/merged_tables/theta_rmse_500.tex <==
% \begin{tabular}{lllll}
%             \toprule
%             & $\hat{\theta}^\text{MUL}_{\text{ELBO}}$ & $\hat{\theta}^\text{DET}_{\text{ELBO}}$ & $\hat{\theta}_{\text{ASMLE}}$ & $\hat{\theta}_{\text{SMLE}}$ \\
%                       \midrule
%             $\theta_1$ & 3.76   & 2.72   & 5.83 & 11.9                         \\
%             $\theta_2$ & 3.20   & 2.07   & 4.64 & 12.6    \\ 
%             \bottomrule
%     \end{tabular}

\begin{tabular}{llll}
\toprule
$B$ &  $\hat{\theta}^\text{PF}_{\text{ELBO}}$ & $\hat{\theta}^\text{DPF}_{\text{ELBO}}$ & $\hat{\theta}_{\text{SMLE}}$ \\ \midrule
1         & 4.86                 & 3.94                 & 16.87                 \\
4          & 4.94                 & 3.37                 & 7.01                  \\
10         & 4.79                 & 2.72                 & 4.53                  \\\bottomrule
\end{tabular}

\begin{tabular}{llll}
\toprule
&  $1$ & $4$ & $10$ \\ \midrule
        & 1.94                 & 2.39                 & 2.8\\
    \bottomrule
\end{tabular}

==> Differentiable_Particle_Filter (arXiv)/tables/theta_diff_MULTINOMIAL_batch_size_4_batch_data_100.tex <==
\begin{tabular}{lr}
\toprule
$\theta_1$ & 0.061 \\
$\theta_2$ & 0.057 \\
\bottomrule
\end{tabular}


==> Differentiable_Particle_Filter (arXiv)/tables/theta_diff_REGULARIZED_batch_size_1_batch_data_100.tex <==
\begin{tabular}{lr}
\toprule
$\theta_1$ & 0.11 \\
$\theta_2$ & 0.11 \\
\bottomrule
\end{tabular}


==> Differentiable_Particle_Filter (arXiv)/tables/theta_diff_REGULARIZED_batch_size_4_batch_data_100.tex <==
\begin{tabular}{lr}
\toprule
$\theta_1$ & 0.052 \\
$\theta_2$ & 0.045 \\
\bottomrule
\end{tabular}


==> tables/MULTINOMIAL_batchsize_100_N_100_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -3.296 & 0.078 \\
                  0.500 & -3.136 & 0.062 \\
                  0.750 & -3.228 & 0.068 \\
\bottomrule
\end{tabular}


==> tables/MULTINOMIAL_batchsize_100_N_25_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -4.068 & 0.177 \\
                  0.500 & -3.801 & 0.169 \\
                  0.750 & -3.896 & 0.176 \\
\bottomrule
\end{tabular}


==> tables/MULTINOMIAL_batchsize_100_N_50_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -3.562 & 0.110 \\
                  0.500 & -3.350 & 0.100 \\
                  0.750 & -3.443 & 0.106 \\
\bottomrule
\end{tabular}


==> tables/REGULARIZED_batchsize_100_N_100_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -3.298 & 0.074 \\
                  0.500 & -3.140 & 0.060 \\
                  0.750 & -3.237 & 0.065 \\
\bottomrule
\end{tabular}


==> tables/REGULARIZED_batchsize_100_N_25_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -4.071 & 0.180 \\
                  0.500 & -3.806 & 0.172 \\
                  0.750 & -3.896 & 0.180 \\
\bottomrule
\end{tabular}


==> tables/REGULARIZED_batchsize_100_N_50_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -3.568 & 0.109 \\
                  0.500 & -3.355 & 0.104 \\
                  0.750 & -3.454 & 0.127 \\
\bottomrule
\end{tabular}


==> tables/VARIANCE_CORRECTED_batchsize_100_N_100_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -3.298 & 0.074 \\
                  0.500 & -3.140 & 0.060 \\
                  0.750 & -3.237 & 0.065 \\
\bottomrule
\end{tabular}


==> tables/VARIANCE_CORRECTED_batchsize_100_N_25_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -4.072 & 0.181 \\
                  0.500 & -3.807 & 0.172 \\
                  0.750 & -3.894 & 0.178 \\
\bottomrule
\end{tabular}


==> tables/VARIANCE_CORRECTED_batchsize_100_N_50_likelihoods_values.tex <==
\begin{tabular}{rrr}
\toprule
 $\theta_1$, $\theta_2$ &   mean &   std \\
\midrule
                  0.250 & -3.568 & 0.109 \\
                  0.500 & -3.355 & 0.104 \\
                  0.750 & -3.454 & 0.126 \\
\bottomrule
\end{tabular}


==> tables/kalman_likelihoods_values.tex <==
\begin{tabular}{rr}
\toprule
 $\theta_1, \theta_2$ &  $\ell(\theta_1, \theta_2)$ \\
\midrule
                0.250 &                      -3.052 \\
                0.500 &                      -2.958 \\
                0.750 &                      -3.015 \\
\bottomrule
\end{tabular}


==> tables/merged_tables/RMSE_optimal_proposal.tex <==

 \begin{tabular}{rrrr}
 \toprule
 & $\ell^\text{ELBO}$ & $\ell^\text{ELBO}_\epsilon$ & $\ell_\epsilon$ \\
 \midrule
  $\text{RMSE}(\phi - \mathbf{1})$ &   0.124 &   0.110 &   0.237\\
 \bottomrule
 \end{tabular}

==> tables/merged_tables/rmse_with_average_smle.tex <==
\begin{table}[H]
    \centering
        \caption{Root mean square error\footnotemark \\ over 50 datasets $/10^{-3}$ }
        \begin{tabular}{llll}
            \toprule
            & $\hat{\theta}^\text{MUL}_{\text{ELBO}}$ & $\hat{\theta}^\text{DET}_{\text{ELBO}}$ & $\hat{\theta}_{\text{Average SMLE}}$ \\
                       \midrule
            $\theta_1$ & 3.76   & 2.72   & 5.83                         \\
            $\theta_2$ & 3.20   & 2.07   & 4.64     \\ 
            \bottomrule
        \end{tabular}
    \label{tab:theta_diff}
\end{table}


==> tables/merged_tables/theta_rmse_500.tex <==
% \begin{tabular}{lllll}
%             \toprule
%             & $\hat{\theta}^\text{MUL}_{\text{ELBO}}$ & $\hat{\theta}^\text{DET}_{\text{ELBO}}$ & $\hat{\theta}_{\text{ASMLE}}$ & $\hat{\theta}_{\text{SMLE}}$ \\
%                       \midrule
%             $\theta_1$ & 3.76   & 2.72   & 5.83 & 11.9                         \\
%             $\theta_2$ & 3.20   & 2.07   & 4.64 & 12.6    \\ 
%             \bottomrule
%     \end{tabular}

\begin{tabular}{llll}
\toprule
$B$ &  $\hat{\theta}^\text{PF}_{\text{ELBO}}$ & $\hat{\theta}^\text{DPF}_{\text{ELBO}}$ & $\hat{\theta}_{\text{SMLE}}$ \\ \midrule
1         & 4.86                 & 3.94                 & 16.87                 \\
4          & 4.94                 & 3.37                 & 7.01                  \\
10         & 4.79                 & 2.72                 & 4.53                  \\\bottomrule
\end{tabular}

\begin{tabular}{llll}
\toprule
&  $1$ & $4$ & $10$ \\ \midrule
        & 1.94                 & 2.39                 & 2.8\\
    \bottomrule
\end{tabular}

==> tables/theta_diff_MULTINOMIAL_batch_size_4_batch_data_100.tex <==
\begin{tabular}{lr}
\toprule
$\theta_1$ & 0.061 \\
$\theta_2$ & 0.057 \\
\bottomrule
\end{tabular}


==> tables/theta_diff_REGULARIZED_batch_size_1_batch_data_100.tex <==
\begin{tabular}{lr}
\toprule
$\theta_1$ & 0.11 \\
$\theta_2$ & 0.11 \\
\bottomrule
\end{tabular}


==> tables/theta_diff_REGULARIZED_batch_size_4_batch_data_100.tex <==
\begin{tabular}{lr}
\toprule
$\theta_1$ & 0.052 \\
$\theta_2$ & 0.045 \\
\bottomrule
\end{tabular}

